Auto Graph Encoder-Decoder for Neural Network Pruning

Model compression aims to deploy deep neural networks (DNN) on mobile devices with limited computing and storage resources. However, most of the existing model compression methods rely on manually defined rules, which require domain expertise. DNNs are essentially computational graphs, which contain rich structural information. In this paper, we aim to find a suitable compression policy from DNNs' structural information. We propose an automatic graph encoder-decoder model compression (AGMC) method combined with graph neural networks (GNN) and reinforcement learning (RL). We model the target DNN as a graph and use GNN to learn the DNN's embeddings automatically. We compared our method with rule-based DNN embedding model compression methods to show the effectiveness of our method. Results show that our learning-based DNN embedding achieves better performance and a higher compression ratio with fewer search steps. We evaluated our method on over-parameterized and mobile-friendly DNNs and compared our method with handcrafted and learning-based model compression approaches. On over parameterized DNNs, such as ResNet-56, our method outperformed handcrafted and learning-based methods with $4.36\%$ and $2.56\%$ higher accuracy, respectively. Furthermore, on MobileNet-v2, we achieved a higher compression ratio than state-of-the-art methods with just $0.93\%$ accuracy loss.

==> Figure_1.tex <==
\begin{figure*}
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
  \includegraphics[width=.9\linewidth]{Figures/Figure1.png}

\end{center}
   \caption{A two-layer hierarchical computation graph. The nodes on the graph denotes the feature maps of input data, and the edges corresponding to primitive operations. In layer 1 (Left),we have three edge types associated with three primitive operations. And each graph in layer 1 corresponding to a compound operation composed of the primitive operations. The computation graphs \{$G^1_{1}$,$G^1_{2}$,$G^1_{3}$\}are becomes the primitive operation in the layer 2. And we can flat the $G^2$ by replacing the edges with computation graphs in layer 1.}


\label{fig:short}
\end{figure*}
